GOALPlace: Begin with the End in Mind

Co-optimizing placement with congestion is integral to achieving high-quality designs. This paper presents GOALPlace, a new learning-based general approach to improving placement congestion by controlling cell density. Our method efficiently learns from an EDA tool's post-route optimized results and uses an empirical Bayes technique to adapt this goal/target to a specific placer's solutions, effectively beginning with the end in mind. It enhances correlation with the long-running heuristics of the tool's router and timing-opt engine -- while solving placement globally without expensive incremental congestion estimation and mitigation methods. A statistical analysis with a new hierarchical netlist clustering establishes the importance of density and the potential for an adequate cell density target across placements. Our experiments show that our method, integrated as a demonstration inside an academic GPU-accelerated global placer, consistently produces macro and standard cell placements of superior or comparable quality to commercial tools. Our empirical Bayes methodology also allows a substantial quality improvement over state-of-the-art academic mixed-size placers, achieving up to 10x fewer design rule check (DRC) violations, a 5% decrease in wirelength, and a 30% and 60% reduction in worst and total negative slack (WNS/TNS).

==> settings/macros.tex <==
\newcommand{\biassquared}{{\textsc{bias}^2}}
\newcommand{\variance}{{\textsc{var}}}
\newcommand{\biassquaredemp}{{\widehat{\textsc{bias}}^2}}
\newcommand{\varianceemp}{{\widehat{\textsc{var}}}}

%\def\deq{\triangleq}
\def\deq{:=}
\newcommand{\reals}{\ensuremath{\mathbb R}}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{\,T}}}} 
\newcommand{\trace}{\mathsf{tr}}
\newcommand{\ind}[1]{\ensuremath{{\mathbf I}{\left\{#1\right\}}}}
\newcommand{\indicator}[1]{\ensuremath{\boldsymbol{1}\left[#1\right]}}
\newcommand{\inner}[1]{\left\langle #1 \right\rangle}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\onehalf}{\ensuremath{\frac{1}{2}}}
\newcommand{\bone}{\ensuremath{\mathbf{1}}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\card}{\mbox{card}}
\renewcommand{\star}{\text{star}}
\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}} \ }
\newcommand{\argmax}[1]{\underset{#1}{\mathrm{argmax}} \ }
\newcommand{\avgni}{\frac{1}{n}\sum_{i=1}^n}
\newcommand{\avgnt}{\frac{1}{n}\sum_{t=1}^n}
\renewcommand{\vec}[1]{\boldsymbol{#1}}

% Expectations and probability
\newcommand{\Ebr}[1]{\mathbb{E}\left\{ #1 \right\}} % curly braces
\newcommand{\En}{\mathbb{E}}  % no brackets or braces
\newcommand{\Es}[2]{\mathbb{E}_{#1}\left[ #2 \right]} % subscript + brackets
\newcommand{\Ps}[2]{\mathbb{P}_{#1}\left[ #2 \right]}
\newcommand{\Prob}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\Eunderone}[1]{\underset{#1}{\E}}
\newcommand{\Eunder}[2]{\underset{\underset{#1}{#2}}{\E}}


% Learning/prediction
\newcommand{\loss}{\mathbf\ell}
\newcommand{\algo}{\widehat{f}}
%\newcommand{\prederm}{\widehat{f}_\text{\tiny erm}}
\newcommand{\prederm}{\widehat{f}_{\scalebox{.4}{erm}}}
\newcommand{\hatf}{\ensuremath{\hat{f}}}
\newcommand{\pred}{\widehat{y}}


\newcommand{\be}{\boldsymbol{e}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}

% Caligraphic and SF
\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
% \cA, \cB, ...
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}

\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
% \sA, \sB, ...
\def\ddef#1{\expandafter\def\csname s#1\endcsname{\ensuremath{\mathsf{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop


\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
% \bA, \bB, ...
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{\mathbf{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\L{{\mathcal{L}}}
\def\N{{\mathcal{N}}}
\def\beqas{\begin{eqnarray*}}
\def\eeqas{\end{eqnarray*}}
\def\beqa{\begin{eqnarray}}
\def\eeqa{\end{eqnarray}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\bit{\begin{itemize}}
\def\eit{\end{itemize}}
\def\ben{\begin{enumerate}}
\def\een{\end{enumerate}}
\def\BA{\begin{array}}
\def\EA{\end{array}}
\def\diag{\mathop{\rm diag}}
\def\mean{\mathop{\rm mean}}
\def\chol{\mathop{\rm chol}}
\def\endmatlab{\mathop{\rm end}}
\def\Diag{\mathop{\rm Diag}}
\def\x{\mathbf{x}}
\def\s{\mathbf{s}}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\Cov}{{\mathop { \rm cov{}}}}
\newcommand{\cov}{{\mathop {\rm cov{}}}}
\newcommand{\corr}{{\mathop { \rm corr{}}}}
\newcommand{\Var}{\mathop{ \rm var{}}}

\newcommand{\var}{\mathop{ \rm var}}
\newcommand{\Tr}{\mathop{ \rm tr}}
\newcommand{\idm}{I}
\newcommand{\rb}{\mathbb{R}}
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof


==> settings/macros_am.tex <==
\usepackage[mathscr]{euscript}
\usepackage{accents}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}

% Copied from mathrsfs.sty
\DeclareSymbolFont{rsfs}{U}{rsfs}{m}{n}
\DeclareSymbolFontAlphabet{\mathscrsfs}{rsfs}

% Probability
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\text{Var}}
\newcommand{\Cov}{\text{Cov}}
%\newcommand{\cN}{\mathcal{N}}

% Sets
%\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\S}{\mathbb{S}}

\def\reals{{\mathbb R}}
\def\ball{{\mathsf B}}

% Variables
\newcommand{\eps}{\varepsilon} 
\newcommand{\vphi}{\varphi}
\def\id{{\mathbf I}}


% Math
\renewcommand{\d}{\textup{d}}
\renewcommand{\l}{\vert}
\newcommand{\dl}{\Vert}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
%\newcommand{\sign}{\text{sign}}
\newcommand{\diag}{\text{diag}}
%\newcommand{\tr}{\text{tr}}
\newcommand{\op}{}
\newcommand{\ones}{\bm{1}}
\newcommand{\what}{\widehat}
\newcommand{\grad}{\nabla}
\def\sT{{\mathsf T}}
\def\bzero{{\boldsymbol 0}}


\def\tu{\tilde{u}}
\def\tg{\tilde{g}}

% Bold symbols
\def\bA{{\boldsymbol A}}
\def\bB{{\boldsymbol B}}
\def\bC{{\boldsymbol C}}
\def\bD{{\boldsymbol D}}
\def\bE{{\boldsymbol E}}
\def\bF{{\boldsymbol F}}
\def\bG{{\boldsymbol G}}

\def\bH{{\boldsymbol H}}
\def\bJ{{\boldsymbol J}}
\def\bK{{\boldsymbol K}}
\def\bL{{\boldsymbol L}}
\def\bM{{\boldsymbol M}}
\def\bO{{\boldsymbol O}}
\def\bP{{\boldsymbol P}}
\def\bQ{{\boldsymbol Q}}
\def\bR{{\boldsymbol R}}
\def\bS{{\boldsymbol S}}
\def\bT{{\boldsymbol T}}
\def\bU{{\boldsymbol U}}
\def\bV{{\boldsymbol V}}
\def\bW{{\boldsymbol W}}
\def\bX{{\boldsymbol X}}
\def\bY{{\boldsymbol Y}}
\def\bZ{{\boldsymbol Z}}

\def\tZ{\tilde{Z}}

\def\tbU{\tilde{\boldsymbol U}}
\def\tbZ{\tilde{\boldsymbol Z}}
\def\tbg{\tilde{\boldsymbol g}}

\def\ba{{\boldsymbol a}}
\def\bb{{\boldsymbol b}}
\def\be{{\boldsymbol e}}
\def\boldf{{\boldsymbol f}}
\def\bg{{\boldsymbol g}}
\def\bh{{\boldsymbol h}}
\def\bi{{\boldsymbol i}}
\def\bj{{\boldsymbol j}}
\def\bk{{\boldsymbol k}}
\def\bt{{\boldsymbol t}}
\def\bu{{\boldsymbol u}}
\def\bv{{\boldsymbol v}}
\def\bw{{\boldsymbol w}}
\def\bx{{\boldsymbol x}}
\def\by{{\boldsymbol y}}
\def\bz{{\boldsymbol z}}

\def\bbeta{{\boldsymbol \beta}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol \eps}}
\def\blambda{{\boldsymbol \lambda}}
\def\bpsi{{\boldsymbol \psi}}
\def\bphi{{\boldsymbol \phi}}
\def\hbtheta{\hat{\boldsymbol \theta}}
\def\hbbeta{\widehat{\boldsymbol \beta}}
\def\hbeta{\widehat{\beta}}
\def\btheta{{\boldsymbol \theta}}
\def\bvphi{{\boldsymbol \vphi}}
\def\bxi{{\boldsymbol \xi}}

\def\bDelta{{\boldsymbol \Delta}}
\def\bLambda{{\boldsymbol \Lambda}}
\def\bPsi{{\boldsymbol \Psi}}
\def\bPhi{{\boldsymbol \Phi}}
\def\bSigma{{\boldsymbol \Sigma}}
\def\bTheta{{\boldsymbol \Theta}}

\def\bfzero{{\boldsymbol 0}}
\def\bfone{{\boldsymbol 1}}



% Symbols with hat
\def\hba{{\widehat {\boldsymbol a}}}
\def\hf{{\widehat f}}
\def\tcT{\widetilde{\mathcal T}}
\def\tK{\widetilde{K}}




% rm symbols
\def\spn{{\rm span}}
\def\supp{{\rm supp}}
\def\Easy{{\rm E}}
\def\Hard{{\rm H}}
\def\post{{\rm post}}
\def\pre{{\rm pre}}
\def\Rot{{\rm Rot}}
\def\Sft{{\rm Sft}}
\def\endd{{\rm end}}
\def\KR{{\rm KR}}
\def\bbHe{{\rm He}}
\def\sk{{\rm sk}}
\def\de{{\rm d}}
\def\He{{\rm He}}
\def\Trace{{\trace}}
\def\lin{{\rm lin}}
\def\res{{\rm res}}
\def\degzero{{\rm deg0}}
\def\degone{{\rm deg1}}
\def\Poly{{\rm Poly}}
\def\Poly{{\rm Poly}}
\def\Coeff{{\rm Coeff}}
\def\de{{\rm d}}
\def\Unif{{\rm Unif}}
\def\He{{\rm He}}
\def\lin{{\rm lin}}
\def\res{{\rm res}}
\def\RF{{\rm RF}}
\def\NT{{\rm NT}}
\def\NF{{\rm NF}}
\def\Cyc{{\rm Cyc}}
\def\RC{{\rm RC}}
\def\kernel{\rm Ker}
\def\image{{\rm Im}}
\def\Easy{{\rm E}}
\def\Hard{{\rm H}}
\def\post{{\rm post}}
\def\pre{{\rm pre}}
\def\Rot{{\rm Rot}}
\def\Sft{{\rm Sft}}
\def\ddiag{{\rm ddiag}}
\def\KR{{\rm KR}}
\def\RR{{\rm RR}}
\def\bbHe{{\rm He}}
\def\eff{{\rm eff}}

\def\spn{{\rm span}}


%mathcal symbols
\def\cV{{\mathcal V}}
\def\cG{{\mathcal G}}
\def\cO{{\mathcal O}}
\def\cP{{\mathcal P}}
\def\cW{{\mathcal W}}
\def\cT{{\mathcal T}}
\def\cC{{\mathcal C}}
\def\cQ{{\mathcal Q}}
\def\cL{{\mathcal L}}
\def\cF{{\mathcal F}}
\def\cE{{\mathcal E}}
\def\cS{{\mathcal S}}
\def\cI{{\mathcal I}}
\def\cV{{\mathcal V}}
\def\cG{{\mathcal G}}
\def\cO{{\mathcal O}}
\def\cP{{\mathcal P}}
\def\cW{{\mathcal W}}
\def\cT{{\mathcal T}}
\def\cH{{\mathcal H}}
\def\cA{{\mathcal A}}



%mathbb mathsf sf symbols
\def\K{{\mathbb K}}
\def\H{{\mathbb H}}
\def\T{{\mathbb T}}
\def\bbV{{\mathbb V}}
\def\W{{\mathbb W}}
\def\sM{{\mathsf M}}
\def\sW{{\mathsf W}}
\def\Unif{{\sf Unif}}
\def\normal{{\sf N}}
\def\proj{{\mathsf P}}
\def\ik{{\mathsf k}}
\def\il{{\mathsf l}}
\def\sM{{\sf M}}
\def\RKHS{{\sf RKHS}}
\def\RF{{\sf RF}}
\def\NT{{\sf NT}}
\def\NN{{\sf NN}}
\def\reals{{\mathbb R}}
\def\integers{{\mathbb Z}}
\def\naturals{{\mathbb N}}
\def\Top{{\mathbb T}}
\def\Kop{{\mathbb K}}
\def\normal{{\sf N}}
\def\proj{{\mathsf P}}
\def\bbV{{\mathbb V}}
\def\sW{{\mathsf W}}
\def\sM{{\mathsf M}}
\def\T{{\mathbb T}}
\def\K{{\mathbb K}}
\def\H{{\mathbb H}}
\def\Unif{{\sf Unif}}
\def\normal{{\sf N}}
\def\Uop{{\mathbb U}}
\def\Hop{{\mathbb H}}
\def\Sop{{\mathbb S}}
\def\proj{{\mathsf P}}
\def\ik{{\mathsf k}}
\def\il{{\mathsf l}}
\def\sM{{\sf M}}
\def\RKHS{{\sf RKHS}}
\def\RF{{\sf RF}}
\def\NT{{\sf NT}}
\def\NN{{\sf NN}}
\def\reals{{\mathbb R}}
\def\integers{{\mathbb Z}}
\def\naturals{{\mathbb N}}
\def\proj{{\mathsf P}}
\def\Hop{{\mathbb H}}
\def\Uop{{\mathbb U}}

\def\oD{\overline{D}}
\def\ta{\tilde{a}}
\def\tR{\tilde{R}}
\def\ttR{\dbtilde{R}}
\def\tba{\tilde{\boldsymbol a}}
\def\bq{{\boldsymbol q}}

\def\hR{\hat{R}}
\def\Lip{{\rm Lip}}
\def\sL{\mbox{\rm\tiny L}}
\def\sNL{\mbox{\rm\tiny NL}}
\def\seff{\mbox{\rm\tiny eff}}
\def\smix{\mbox{\rm\tiny mix}}
\def\seq{\mbox{\rm\tiny seq}}
\def\slin{\mbox{\rm\tiny lin}}
\def\sTV{\mbox{\rm\tiny TV}}
\def\sGF{\mbox{\rm\tiny GF}}
\def\samp{\mbox{\rm\tiny s}}
\def\wid{\mbox{\rm\tiny w}}
\def\of{\overline{f}}
\def\obtheta{\overline{\boldsymbol \theta}}
\def\stest{\mbox{\tiny\rm test}}

\def\ERM{{\rm ERM}}
\def\Sp{{\mathbb S}}
\def\oalpha{\overline{\alpha}}
\def\hE{\widehat{{\mathbb E}}}
\def\hh{\hat{h}}
\def\tih{\tilde{h}}

\def\oby{\overline{\boldsymbol y}}
\def\br{{\boldsymbol r}}
\def\bfe{{\boldsymbol e}}
\def\bff{{\boldsymbol f}}

\def\oq{\overline{q}}

\def\tlambda{\tilde{\lambda}}

\def\ratio{\zeta}


\usepackage{color}

\newcommand{\am}[1]{\noindent{{\color{red}\textbf{\#\#\# AM:}
\textsf{#1} \#\#\#}}}

\def\cuB{\mathscrsfs{B}}
\def\cuV{\mathscrsfs{V}}

\def\SNR{{\sf SNR}}
\def\rank{{\rm rank}}
\def\hbK{\hat{\boldsymbol K}}
\def\hrho{\widehat{\rho}}

\def\eval{s}
\def\Eval{{\boldsymbol S}}

\def\uF{\underline{F}}
\def\ulambda{\underline{\lambda}}
\def\Risk{{L}}
\def\hRisk{\widehat{L}}

